Design and Analysis of High Performance Heterogeneous Block-based Approximate Adders

Approximate computing is an emerging paradigm to improve the power and performance efficiency of error-resilient applications. As adders are one of the key components in almost all processing systems, a significant amount of research has been carried out towards designing approximate adders that can offer better efficiency than conventional designs, however, at the cost of some accuracy loss. In this paper, we highlight a new class of energy-efficient approximate adders, namely Heterogeneous Block-based Approximate Adders (HBAA), and propose a generic configurable adder model that can be configured to represent a particular HBAA configuration. An HBAA, in general, is composed of heterogeneous sub-adder blocks of equal length, where each sub-adder can be an approximate sub-adder and have a different configuration. The sub-adders are mainly approximated through inexact logic and carry truncation. Compared to the existing design space, HBAAs provide additional design points that fall on the Pareto-front and offer a better quality-efficiency trade-off in certain scenarios. Furthermore, to enable efficient design space exploration based on user-defined constraints, we propose an analytical model to efficiently evaluate the Probability Mass Function (PMF) of approximation error and other error metrics, such as Mean Error Distance (MED), Normalized Mean Error Distance (NMED) and Error Rate (ER) of HBAAs. The results show that HBAA configurations can provide around 15% reduction in area and up to 17% reduction in energy compared to state-of-the-art approximate adders.

==> Tex_Files/CLA_16_bit_Power.tex <==
\begin{table}[h]
  \centering
  \caption{Accuracy of our proposed estimation model for computing Power of 16-bit CLA configurations}
   \adjustbox{max width=\columnwidth}{%
    \begin{tabular}{|c|c|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|}
    \hline
    16-bit Adder & Block size & Power Estimate using the proposed analytical Model ($\mu W$) & Power computed using Synopsys PrimeTime ($\mu W$) & Accuracy of power estimation model \\ \hline
    \multirow{4}{*}{CLA} 
    & 2 & 6723.36 &	7028.24&	95.66\% \\\cline{2-5}
      & 4 & 7203.6&	7812.18&	92.21\%\\\cline{2-5}
      & 8 & 11327.4&	12387.64&	91.44\%\\\hline
    \end{tabular}}%
  \label{tab:hardware_power_16_CLA}%
\end{table}


==> Tex_Files/CLA_16_bit_area.tex <==
\begin{table}[h]
  \centering
  \caption{Accuracy of our proposed estimation model for computing Area of 16-bit CLA configurations}
   \adjustbox{max width=\columnwidth}{%
    \begin{tabular}{|c|c|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|}
    \hline
    16-bit Adder & Block size & Area Estimate using the proposed analytical Model  ($\mu m^2$)&	Area computed using Synopsys Design Compiler  ($\mu m^2$)& 	Accuracy of area estimation model \\ \hline
    \multirow{4}{*}{CLA} 
    & 2 & 23.52 &	25.26&	93.11\% \\\cline{2-5}
      & 4 & 25.2&	27.27&	92.41\%\\\cline{2-5}
      & 8 & 26.04&	28.29&	92.05\%\\\hline
    \end{tabular}}%
  \label{tab:hardware_area_16_CLA}%
\end{table}


==> Tex_Files/CLA_16_bit_delay.tex <==
\begin{table}[h]
  \centering
  \caption{Accuracy of our proposed estimation model for computing Delay of 16-bit CLA configurations}
   \adjustbox{max width=\columnwidth}{%
    \begin{tabular}{|c|c|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|}
    \hline
    16-bit Adder & Block size & Delay Estimate using the proposed analytical Model ($nSec$) & Delay computed using Synopsys Design Compiler ($nSec$) & Accuracy of delay estimation model \\ \hline
    \multirow{4}{*}{CLA} 
    & 2 & 27.72 &	28.86&	96.05\% \\\cline{2-5}
      & 4 & 27.72&	30.03&	92.31\%\\\cline{2-5}
      & 8 & 42.84&	37.39&	85.42\%\\\hline
    \end{tabular}}%
  \label{tab:hardware_delay_16_CLA}%
\end{table}


==> Tex_Files/Error_accuracy.tex <==
\begin{table}[ht]
  \centering
  \caption{Accuracy of our proposed analytical model for computing MED of HBAA configurations}
   \adjustbox{max width=\columnwidth}{%
    \begin{tabular}{|c|c|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|}
    \hline
    Adder & Configuration & MED calculation using Monte Carlo Simulation &  MED calculation using Analytical Model & Accuracy of the Analytical Model \\ \hline
    \multirow{15}{*}{16-bit HBAA} 
    & \{3,2,4,1\}\{1,3,0,4\} & 7043.946 & 7245.68 & 97.22\% \\\cline{2-5}
      & \{4,2\}\{0,2\} & 66.54 &	66.75 & 99.69\% \\\cline{2-5}
      &\{2,2,2,1\}\{0,0,0,1\} & 62.864 & 63.25 &	99.39\% \\\cline{2-5}
        &\{6\}\{3\} & 11.869 &	11.875 &	99.95\% \\\cline{2-5}
        &\{2,1,2,1,0,2,1,1\}\{1,1,2,1,2,1,2,2\} &9991.92 &	10801.6&	92.50\% \\\cline{2-5}
        &\{3,2,3\}\{2,2,1\} &358.413	& 358.875	&99.87\%\\\cline{2-5}
        &\{4,4\}\{0,2\} & 58.97&	59.628	&98.90\%\\\cline{2-5}
        &\{5,2\}\{4,4\}  & 1486.24	&1567.38&	94.82\%\\\cline{2-5}
        &\{2,1,2,1,0,2\}\{0,0,0,1,2,1\} & 1042.74	&1093.92&	95.32\% \\\cline{2-5}
        &\{2,2,2,2,1,2,2\}\{1,0,2,1,2,2,1\}	&2812.96	&2945.124&	95.51\% \\\cline{2-5}
        &\{2,3\}\{0,4\} & 108.12	&109.75	&98.51\% \\\cline{2-5}
        &\{1,1,2,0,0,2\}\{0,1,1,1,2,0\}	&667.34	&675.105	&98.85\%\\\cline{2-5}
        &\{4,4\}\{2,3\}	& 60.53	&60.61	&99.87\% \\\cline{2-5}
        &\{2,1,2,1,0,2\}\{1,1,0,1,2,1\} & 1354.68	&1380.75	&98.11\%\\\cline{2-5}
        &\{2,1,2,1,2,2,1,1\}\{1,2,2,1,2,0,2,2\} &10463.76&	10912.65&	95.89\%\\\hline
        \multirow{6}{*}{32-bit HBAA}   & \{[4,4,4,2][0,0,0,2]\} & 4095.66  &  4095.75 &99.99\%  \\\cline{2-5}
       & \{[4,2][0,2]\} & 15.75 & 15.75 &100\%  \\\cline{2-5}
       & \{[4,1][0,3]\} & 7.7543  & 7.75 &99.94\%  \\\cline{2-5}
      & \{[4,4,4,1][0,0,0,3]\} & 2048.23 & 2047.75 & 99.97\% \\\cline{2-5}
      & \{[4,4,4,2][0,0,0,3]\} & 3071.39 & 3071.98  & 99.98\% \\\cline{2-5}
     & \{[4,4,4,4,1][0,0,0,0,3]\} & 32750.77&31867.75&97.22\%\\\hline
    \end{tabular}}%
  \label{tab:error_16_32}%
\end{table}


==> Tex_Files/HBAA_16_CLA_Power.tex <==
\begin{table}[h]
  \centering
  \caption{Accuracy of our proposed estimation model for computing the Power of 16-bit approximate adders}
   \adjustbox{max width=\columnwidth}{%
    \begin{tabular}{|c|c|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|}
    \hline
    16-bit Adder & Configuration & Power Estimate using the proposed analytical Model ($\mu W$) & Power computed using Synopsys PrimeTime ($\mu W$) & Accuracy of power estimation model \\ \hline
    \multirow{8}{*}{HBAA} 
      & \{0,4\}\{8,4\} & 8647.8 & 8852.3 & 97.69\% \\\cline{2-5}
      & \{3,2,4,1\}\{1,3,0,4\} & 2691.78 & 3121.3 & 86.24\% \\\cline{2-5}
      &\{3,2,3\}\{2,2,1\} & 3339.06 & 3926.5 & 85.04\% \\\cline{2-5}
        &\{4,4\}\{0,2\} & 4129.02 & 4532.5 & 91.10\% \\\cline{2-5}
        &\{4\}\{2\}  & 6163.08 & 6974.8 & 88.36\% \\\cline{2-5}
        &\{2,1,2,1,2\}\{0,0,0,1,1\} & 2322.9 & 2562.3 & 90.66\% \\\cline{2-5}
        &\{2,2,2,2,1,2,2\}\{1,0,2,1,2,2,1\}	& 1914 & 2138.6 & 89.50\% \\\hline

    \end{tabular}}%
  \label{tab:hardware_power_16}%
\end{table}

==> Tex_Files/HBAA_16_CLA_delay.tex <==
\begin{table}[h]
  \centering
  \caption{Accuracy of our proposed estimation model for computing the Delay of 16-bit approximate adders}
   \adjustbox{max width=\columnwidth}{%
    \begin{tabular}{|c|c|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|}
    \hline
    16-bit Adder & Configuration & Delay Estimate using the proposed analytical Model ($nSec$) & Delay computed using Synopsys Design Compiler ($nSec$) & Accuracy of delay estimation model \\ \hline
    \multirow{8}{*}{HBAA} 
      & \{0,4\}\{8,4\} & 42.84 & 38.27 & 88.06\% \\\cline{2-5}
      & \{3,2,4,1\}\{1,3,0,4\} & 20.16 & 22.18 & 90.89\% \\\cline{2-5}
      &\{3,2,3\}\{2,2,1\} & 22.68 & 24.81 & 91.41\% \\\cline{2-5}
        &\{4,4\}\{0,2\} & 25.2 & 28.13 & 89.58\% \\\cline{2-5}
        &\{4\}\{2\}  & 27.72 & 30.03 & 92.31\% \\\cline{2-5}
        &\{2,1,2,1,2\}\{0,0,0,1,1\} & 17.64 & 20.06 & 87.94\% \\\cline{2-5}
        &\{2,2,2,2,1,2,2\}\{1,0,2,1,2,2,1\}	& 12.6 & 14.61 & 86.24\% \\\hline

    \end{tabular}}%
  \label{tab:hardware_delay_16}%
\end{table}

==> Tex_Files/HBAA_CLA_16_area.tex <==
\begin{table}[h]
  \centering
  \caption{Accuracy of our proposed estimation model for computing the Area of 16-bit approximate adders}
   \adjustbox{max width=\columnwidth}{%
    \begin{tabular}{|c|c|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|}
    \hline
    16-bit Adder & Configuration & Area Estimate using the proposed analytical Model ($\mu m^2$) & Area computed using Synopsys Design Compiler ($\mu m^2$) & Accuracy of area estimation model \\ \hline
    \multirow{8}{*}{HBAA} 
      & \{0,4\}\{8,4\} & 19.88 & 22.26 & 89.31\% \\\cline{2-5}
      & \{3,2,4,1\}\{1,3,0,4\} & 12.74 & 13.57 & 93.88\% \\\cline{2-5}
      &\{3,2,3\}\{2,2,1\} & 14.14 & 15.63 & 90.47\% \\\cline{2-5}
        &\{4,4\}\{0,2\} & 15.82 & 16.94 & 93.39\% \\\cline{2-5}
        &\{4\}\{2\}  & 21.56 & 23.41 & 92.10\% \\\cline{2-5}
        &\{2,1,2,1,2\}\{0,0,0,1,1\} & 12.46 & 13.82 & 90.16\% \\\cline{2-5}
        &\{2,2,2,2,1,2,2\}\{1,0,2,1,2,2,1\}	& 14 & 15.4 & 90.91\% \\\hline

    \end{tabular}}%
  \label{tab:hardware_area_16}%
\end{table}
